Quantum Fourier Transformation Circuits Compilation

In this research paper, our primary focus revolves around the domain-specific hardware mapping strategy tailored for Quantum Fourier Transformation (QFT) circuits. While previous approaches have heavily relied on SAT solvers or heuristic methods to generate hardware-compatible QFT circuits by inserting SWAP gates to realign logical qubits with physical qubits at various stages, they encountered significant challenges. These challenges include extended compilation times due to the expansive search space for SAT solvers and suboptimal outcomes in terms of the number of cycles required to execute all gate operations efficiently. In our study, we adopt a novel approach that combines technical intuition, often referred to as "educated guesses," and sophisticated program synthesis tools. Our objective is to uncover QFT mapping solutions that leverage concepts such as affine loops and modular functions. The groundbreaking outcome of our research is the introduction of the first set of linear-depth transformed QFT circuits designed for Google Sycamore, IBM heavy-hex, and the conventional 2-dimensional (2D) grid configurations, accommodating an arbitrary number of qubits denoted as 'N'. Additionally, we have conducted comprehensive analyses to verify the correctness of these solutions and to develop strategies for handling potential faults within them.

==> 2d.tex <==














\section{Linear-depth QFT on 2D Grid}

\subsection{Unit Definition}

 We consider each row in the 2D grid as a unit and place qubits in natural number ordering from left to right, and from top row to bottom row. This is a row-major order initial layout. Similar to Google Sycamore, the problem could be solved by tackling three sub-problems: intra-unit interaction QFT-IA, inter-unit interaction QFT-IE, and unit swapping.

%subsection{Unit SWAP}
%\vspace{-3pt}
% \emph{The unit SWAP in 2D Grid:} 
The unit swap is trivial by applying transversal SWAPs using the vertical links between two units in one step.
% It happens in one time step.
\vspace{-5pt}

\subsection{Intra-unit and inter-unit QFT}

\paragraph{Intra-unit QFT}
The structure of a single unit is exactly the same as the LNN structure. We leverage the existing solution for QFT on LNN for QFT-IA.



\textbf{The intuition for inter-Unit QFT}
The intuition is contrary to that of the inter-unit in Google Sycamore. Recall that we ``guessed" in Google Sycamore, that the top row and bottom should move in sync, but now this should not work.   

If we look at path crossing in Fig. \ref{fig:pathcross}, now the two qubits on the top row and bottom row should meet at exactly the same column, as opposed to two columns of distance 1. This is because a 2D grid has direct vertical links between qubits in the top row and the bottom row. 

In this case, the top-row qubits and bottom-row qubits should not move in the same way. Otherwise, for any column at any time instant, the top qubit's neighbor in the bottom row is always the same. This makes it impossible to do all-to-all interaction between these two rows.

Now our guess is that each qubit should still travel along a path, but there must be a difference between the starting points of movement (SWAPs) in the top row and the bottom row. Two qubits on different rows will have their paths cross at some point (meeting in the same column).  This leads to our program synthesis model as follows. 


\subsection{Program Synthesis for This Architecture}

\paragraph{Specification}

The specification is similar to that in Google Sycamore. The only difference is that we do not exclude the qubit pairs in the vertical links at initial qubit mapping.  



     

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.3\textwidth]{figs/pathcross_strict_2D.pdf}
    \caption{Trajectory of two points from the top row and the bottom row.}
    \label{fig:pathcross}
\end{figure}













\textbf{Implementation.} With the above conditions, our formulated code shape is in Fig. \ref{fig:syn2dIE}.  

\begin{figure}[htb]
    \centering
\includegraphics[width=0.45\textwidth]{figs/syn2dIE.pdf}
    \caption{Synthesized code for inter-unit of the 2D regular grid in the strict version. }
    \label{fig:syn2dIE}
\end{figure}

In the code in Fig. \ref{fig:syn2dIE}, ``beg\_u" and ``end\_u" respectively represent the begin and end location for the SWAPs in the top row. ``beg\_d" and ``end\_d" respectively represent the begin and end locations for the SWAPs in the bottom row. CPHASE gates operate on a range of vertical links, and the range is a linear function of the loop induction and loop invariant variables too. $m$ is the unit size.

We specifically add a difference between the starting location of the top-row SWAP, and that of the bottom-row SWAP, using the modular function ``beg\_u + ??" mod 2.  We simplified the loop by fixing the movement of the top-row as that in QFT LNN. In this case, the simple code shape actually worked. It found a solution successfully, shown in Fig. \ref{fig:syn2dIE} (b). 

We took a step further and chose not to fix the movement in the top row. Rather, we use piecewise linear functions to specify the beginning and ending locations for intra-row SWAP, as shown in Fig. \ref{fig:syn2drelaxed}. Using this approach, we found a solution for QFT-IE-relaxed as shown in Fig. \ref{fig:syn2drelaxed} (b). The repeated step is visualized in Fig. \ref{fig:QFT-IE-Sycamore-strict-relaxed} (b). 




 
 

\begin{figure}[htb]
    \centering
    \vspace{-7pt} \includegraphics[width=0.47\textwidth]{figs/syn2dIE_relaxed.pdf}
    \vspace{-5pt}
    \caption{2-unit interaction for the relaxed order QFT-IE.}
    \label{fig:syn2drelaxed}
    \vspace{-0.1in}
\end{figure}








































 



\begin{comment}

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.35\textwidth]{figs/IE_2D_strict&relax.pdf}
    \caption{The repeated steps of QFT-IE-strict and QFT-IE-relaxed in inter-unit 2D grid. Note that the starting point for the top row is set to 0, in this example, but it in fact alternates between 0 and 1. We do not show them here due to the space limit. The bottom row alternates with the top row.}
    \label{fig:2dinterrepeat}
\end{figure}
\vspace{-5pt}
% Repeat in the order of transition 1, 2, 3, and 4 until all CPHASE gates complete execution.
\end{comment}





\vspace{-0.1in}
\subsection{Time Complexity}

As for the time complexity, we use unit QFT on a line, as shown in Fig. \ref{fig:unitQFTline}. Assuming we have $N=m*m$ qubits. Each unit has $m$ qubits. 

\textbf{\emph{QFT-IE-Relaxed}} Each QFT-IA has complexity $4m-6$. Each QFT-IE has complexity $2m$. Each unit SWAP takes one time step. There are $m + O(1)$ QFT-IE steps. There are $m+O(1)$ mixed (QFT-IA, QFT-IE) steps. In total, the complexity is $6m^2 + O(m) = 6N + O(\sqrt{N})$.

\textbf{\emph{QFT-IE-Strict}} Since the strict version doubles the time complexity compared with the relaxed version. The overall complexity is $8N + O(\sqrt{N})$



==> TODO.tex <==
Xiangyu:
1. to check whether we can add beg/end into LNN, instead of brute-force solution
2. Neutral atom(Geyser paper):
https://dl.acm.org/doi/10.1145/3470496.3527428
3. priorities are list in Xmind.


==> correctness.tex <==
\section{Correctness}
\label{sec:verification}
Correctness is the first priority. We should to guarantee the outcome follows the dependency to complete all gate operations in QFT. 

Ideally, we should provide a formal proof for the correctness of our implementation. As for one type of architecture, our solution should work for all concrete configurations determined by parameter m. This will involve proofs in symbolic format. 

In fact, we take a step back to do simulation using python script, which simulates all gate operations in each step. 
We wrote a python script~\cite{simulation_script} to simulate the QFT process, including gate operations and SWAP operations. Then, we check 2 main points: do all gate operations follow the dependency constraints in QFT and do we complete all necessary QFT gate operations? We believe this is sufficient in our current setting because we have already covered quite large number of qubits (1600 qubits), more than the largest quantum machines~\cite{largest_quantum_machine}.
Until now, we have not yet found any incorrectness.
We leave the formal proof of the correctness of our program into future work.

 As for the other 2 benchmarks (satmap and sabre), we did not develop them from scratch so we have no control over the code base. Instead, we do a manual check of their outcome when the size is small and assume they can work as well for larger sizes. Currently, there is nothing wrong with their output either.


==> neutralatom.tex <==
\section{Neutral-atom}
\xiangyu{Check whether the correctness of the neutral atom description}
Neutral-atom architecture: Multiple quantum computing technologies are rapidly emerging including superconducting qubit, neutral atom, trapped ion, and photon. It is likely that different users will choose various technologies to exploit the specific advantage of each type for running their customized quantum program. Due to the fact that it is a relatively new structure, we will describe in detail the neutral-atom in this subsection.

Compared with superconducting-qubit quantum computer, neutral atom qubits are entangled using Rydberg interactions instead of physical links. Therefore, an important feature of neutral-atom quantum computing is called the interaction radius or the restriction zone, determining which qubits are active at a particular stage. Specifically, it uses a circle to represent the Rydberg influence range. While a multi-qubit gate is being performed, other qubits that are within the Rydberg influence range cannot run any other gates.

For example, in Fig.~\ref{fig:neutral_atom}, qubits are arranged in a triangular topology, where the restriction zones are represented by a circle with radius to be 2. When there are two active gates executing ($q_6$ and $q_7$, $q_9$ and $q_10$), all other qubits within the restriction zone must keep inactive. For instance, when $q_6$ and $q_7$ are executing a gate, $q_8$ cannot get involved in any other gate operations.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/neutral_atom_arch.pdf}
    \caption{The structure of netural atom. }
    \label{fig:neutral_atom}
\end{figure}

Intra-unit QFT solution: The intra-unit QFT solution in neutral-atom architecture is quite similar to that LNN because all qubits are chained in a line. 
In comparison, the major differences are related to the restriction zone represented by a circle. Therefore, we cannot complete either one SWAP step or one CPHASE step in LNN within one step in neutral-atom setting. One way to tackle this issue is to divide it into multiple steps, each of which will complete partial SWAP/CPHASE gate operations. 

Just as the example shown in Fig.~\ref{fig:neutral_atom_intra}. Here we assume the radius of the restriction zone in neutral-atom structure is 2. In order to complete gate operations between $q_0$ and $q_1$, $q_2$ and $q_3$, $q_4$ and $q_5$, we have to use 2 steps to guarantee that each step, no more than 1 qubits in a restriction zone are actively involved in multi-qubit gate operations.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth]{figs/neutral_atom_intra.pdf}
    \caption{Intra-unit CPHASE/SWAP in neutral atom.}
    \label{fig:neutral_atom_intra}
\end{figure*}


Inter-unit QFT solution: The solution for inter-unit QFT can be inherited with modification from the solution from 2D grid as well. Specifically, there are a lot of similarities between neutral-atom and 2D grid architecture because any ith qubit above is connected to the ith qubit below. In addition, the ith qubit above, except the first and the last qubit in a row, is also connected to the (i-1)th and (i+1)th qubit below. In terms of the connectivity, neutral-atom is a superset of 2D grid. Therefore, we want to transplant the solution from 2D grid to netural-atom. 
However, we still need to obey the rule which limits the number of qubits involving in multi-qubit gate operations within a restriction zone to be at most 1. Accordingly, either one CPHASE step or one SWAP step should be divided into multiple steps in this setting.

For example, assuming the radius of restriction zone to be 2, we visualize the inter-unit process of neutral-atom in Fig.~\ref{fig:neutral_atom_swap} and Fig.~\ref{fig:neutral_atom_cphase}. As for the SWAP, for each row, we cannot do consecutive SWAPs for all qubits in one cycle so we need to divide it into 2 steps; in addition, we cannot do swap for one row if its adjacent row is executing some qubit SWAPs. This forces us to separate the swap of different rows into different cycles. As for the CPHASE, we could complete the CPHASE between 2 units in 2 cycles, each cycle will focus on implementing CPHASE gates over qubits with even number and qubits with odd number respectively.

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth]{figs/neutral_atom_swap.pdf}
    \caption{Inter-unit SWAP in neutral atom.}
    \label{fig:neutral_atom_swap}
\end{figure*}

\begin{figure*}[htb]
    \centering
    \includegraphics[width=\textwidth]{figs/neutral_atom_cphase.pdf}
    \caption{Inter-unit CPHASE in neutral atom.}
    \label{fig:neutral_atom_cphase}
\end{figure*}

\xiangyu{Ask Eddy: do we need to add the affine for loop here?}

==> tech.tex <==





